PocketRL: Training a 7B Language Model with Reinforcement Learning on One RTX 5090

It is now common to post-train large language models with reinforcement learning with verifiable rewards (RLVR), but its heavy memory use, and hence high cost, is an important bottleneck for RLVR research and a major expense in training frontier models. We introduce PocketRL, a low-cost, memory-efficient RLVR code base that trains a 7B model on a single RTX 5090 and a 27B model on only four, without CPU offloading. PocketRL combines two ideas. First, we project each layer's gradient and optimizer state onto a small basis fitted to the layer's input activations by a QR factorisation, which we call ActGRA, and show that such a basis retains far more of the gradient than the random projections used in prior work. Second, we propose training on 16-bit weights with half an extra byte per weight that carries the rounding error, which prevents small updates from being lost. The same 16-bit weights are used for inference, which saves further memory. Together, these methods reduce memory use for training a 7B model by 84%. This enables us to train a competitive 7B model in less than 8 hours on a single RTX 5090 for just $4.71, less than 9% of the cost of training comparable models. PocketRL also reduces the cost of a 27B training step by more than 77% compared with similar code bases. We open-source our PocketRL code base.

==> table_greedy.tex <==
\begin{table}[H]
\centering
\caption{\textbf{Accuracy on test sets using greedy decoding.} We report greedy accuracy (\%) as the mean (standard error) over three training seeds at the last step. We trained all fine-tuned models in \sys{}.}
\label{tab:greedy-endpoints}
\small
\setlength{\tabcolsep}{3pt}
\begin{tabular}{@{}lrrrrrrr@{}}
\toprule
Method & \shortstack{Math\\500} & \shortstack{AIME\\2024} & \shortstack{AIME\\2025} & \shortstack{AMC\\2023} & \shortstack{Minerva\\Math} & \shortstack{Olympiad\\Bench} & Average \\
\midrule
\multicolumn{8}{@{}l}{\textbf{Qwen2.5-Math-1.5B}} \\
Base model & 34.8 & 10.0 & 0.0 & 25.0 & 8.5 & 23.3 & 16.9 \\
Dense & 69.3 (0.6) & \textbf{20.0 (0.0)} & 10.0 (1.9) & 47.5 (2.5) & 26.2 (0.6) & 34.4 (0.7) & 34.6 (0.3) \\
LoGRA & 70.3 (0.7) & 11.1 (2.9) & 6.7 (1.9) & 48.3 (2.2) & \textbf{28.4 (0.3)} & 35.4 (0.5) & 33.4 (0.7) \\
ActGRA & \textbf{72.3 (0.4)} & 13.3 (1.9) & \textbf{12.2 (2.9)} & \textbf{50.8 (4.4)} & 27.3 (0.3) & \textbf{36.0 (0.3)} & \textbf{35.3 (1.0)} \\
\midrule
\multicolumn{8}{@{}l}{\textbf{Qwen2.5-Math-7B}} \\
Base model & 50.0 & 13.3 & 6.7 & 45.0 & 11.4 & 18.4 & 24.1 \\
Dense & 79.1 (0.9) & 24.4 (4.0) & 8.9 (1.1) & 60.0 (3.8) & 34.7 (0.8) & 41.4 (0.9) & 41.4 (1.3) \\
LoGRA & 77.9 (0.9) & 25.6 (1.1) & \textbf{14.4 (2.2)} & \textbf{69.2 (2.2)} & 34.9 (2.0) & \textbf{43.4 (0.1)} & \textbf{44.2 (0.9)} \\
ActGRA & \textbf{80.0 (0.7)} & \textbf{27.8 (4.4)} & 11.1 (1.1) & 61.7 (4.6) & \textbf{36.8 (1.1)} & 43.2 (0.5) & 43.4 (0.7) \\
\midrule
\multicolumn{8}{@{}l}{\textbf{Qwen3.8-27B}} \\
ActGRA & 94.2 (1.0) & 57.8 (1.1) & 48.9 (1.1) & 86.7 (4.4) & 49.9 (1.6) & 64.0 (0.5) & 66.9 (0.6) \\
\bottomrule
\end{tabular}
\end{table}

